SetVAE: Learning Hierarchical Composition for Generative Modeling of Set-Structured Data

Generative modeling of set-structured data, such as point clouds, requires reasoning over local and global structures at various scales. However, adopting multi-scale frameworks for ordinary sequential data to a set-structured data is nontrivial as it should be invariant to the permutation of its elements. In this paper, we propose SetVAE, a hierarchical variational autoencoder for sets. Motivated by recent progress in set encoding, we build SetVAE upon attentive modules that first partition the set and project the partition back to the original cardinality. Exploiting this module, our hierarchical VAE learns latent variables at multiple scales, capturing coarse-to-fine dependency of the set elements while achieving permutation invariance. We evaluate our model on point cloud generation task and achieve competitive performance to the prior arts with substantially smaller model capacity. We qualitatively demonstrate that our model generalizes to unseen set sizes and learns interesting subset relations without supervision. Our implementation is available at https://github.com/jw9730/setvae.

==> cvpr_draft/conclusion.tex <==
% !TEX root = cvpr.tex
\vspace*{-0.05in}
\section{Conclusion}
\label{sec:conclusion}
\vspace*{-0.05in}
% \cutsectiondown
%{\fontfamily{cmss}\selectfont\color{blue}[TODO: Write conclusion]}
%SetVAE learn a generative model by VAE, and achieves exchangeability by stacking permutation equivariant ABLs, which are variant of ISAB. Furthermore, SetVAE learns subset reasoning as a product of hierarchical latent modeling. As a result, SetVAE yields better results than prior state-of-the-arts methods with a few parameters.
We introduced SetVAE, a novel hierarchical VAE for sets of varying cardinality. By adopting a novel bottleneck equivariant layer that exploits subset representations, SetVAE performs hierarchical subset reasoning to encode and generate sets in a coarse-to-fine manner. As a result, SetVAE generates high-quality, diverse sets using a less number of parameters than baselines. We also showed that SetVAE achieves cardinality disentanglement and generalization. Our future work could include extending SetVAE to datasets involving sparse object annotations.


==> cvpr_draft/experiment.tex <==
% !TEX root = cvpr.tex
\section{Experiments}
\label{sec:experiment}
% This section discusses evaluation results of SetVAE.
% See the supplementary file for more results and training details.

\iffalse
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/comparison-ablation.pdf}
    \caption{Examples of randomly generated samples from SetVAE (ours) and PointFlow in ShapeNet. 
    \shcmt{Consider different way to visualize the points.}
    \shcmt{Remove comparison to PointFlow and make it to single column.}
    }
\end{figure*}
\fi

\begin{figure}[t!]
    \centering
    % \vspace{-0.3cm}
    \includegraphics[width=0.47\textwidth]{figures/fig-4-comparison.pdf}
    \vspace{-0.5cm}
    \caption{Examples of randomly generated point sets from SetVAE (ours) and PointFlow in ShapeNet. 
    }
    \label{fig:compare_pointflow}
    \vspace{-0.5cm}
\end{figure}

\subsection{Experimental Setup}
\label{sec:quantitative}
\paragraph{Dataset}
We examine SetVAE using ShapeNet~\cite{chang2015shapenet}, Set-MNIST~\cite{zhang2020deep}, and Set-MultiMNIST~\cite{eslami2016attend} datasets.
For ShapeNet, we follow the prior work using 2048 points sampled uniformly from the mesh surface~\cite{yang2019pointflow}. %, normalized to axis-wise zero mean and unit variance \cite{yang2019pointflow}.
% For Set-MNIST, we binarized the pixel values of MNIST by mean value over the training set and scale the coordinates to $[0, 1]$ \cite{kosiorek2020conditional}.
For Set-MNIST, we binarized the images in MNIST and scale the coordinates to $[0, 1]$ \cite{kosiorek2020conditional}.
%For Set-MNIST, we binarized the pixel values of MNIST and scale the coordinates to $[0, 1]$ \cite{kosiorek2020conditional}.
Similarly, we build Set-MultiMNIST using $64\times64$ images of MultiMNIST~\cite{eslami2016attend} with two digits randomly located without overlap.
%To avoid data spoiling, we use the MNIST training set to build the training set of MultiMNIST and use the MNIST validation set to build the validation set of MultiMNIST.

\cutparagraphup
\paragraph{Evaluation Metrics}
% To evaluate ShapeNet generation performance, we use Jensen-Shannon Divergence (JSD), Minimum Matching Distance (MMD), Coverage (COV), and 1-Nearest Neighbor Accuracy (1-NNA) as evaluation metrics.
For evaluation in ShapeNet, we compared the standard metrics including Jensen-Shannon Divergence (JSD), Minimum Matching Distance (MMD), Coverage (COV), and 1-Nearest Neighbor Accuracy (1-NNA), where the similarity between point clouds required to compute those metrics are evaluted using both Chamfer Distance (CD) and Earth Mover's Distance (EMD).
%To compute the metrics, we use both Chamfer Distance (CD) and Earth Mover's Distance (EMD) to measure the similarity between point clouds.
The details of the metrics can be found in the supplementary file.

% \cutparagraphup
\subsection{Comparison to Other Methods}
We compare SetVAE with the state-of-the-art generative models for point clouds including l-GAN~\cite{achlioptas2018learning}, PC-GAN~\cite{li2018point}, and PointFlow~\cite{yang2019pointflow}.
Following these works, we train our model for each category of airplane, chair, and car.
% Following these works, we train one SetVAE per a category on airplane, chair, and car from the ShapeNet dataset \cite{chang2015shapenet}.

Table~\ref{table:pointeval} summarizes the evaluation result.
SetVAE achieves better or competitive performance to the prior arts using a \emph{much smaller} number of parameters ($6\%$ to $33\%$ of competitors).
% SetVAE substantially yields better results than prior state-of-the-art with only 6\%-33\% of their number of parameters.
Notably, SetVAE outperforms PointFlow with a significant margin in terms of coverage (COV) and has better or comparable minimum matching distance (MMD).
High coverage indicates that SetVAE generates diverse samples covering various modes in data, and low MMD implies that it generates consistent and high-quality samples.
Together, the results indicate that SetVAE generates diverse, high-quality point sets.
Notably, we find that SetVAE trained with CD (Eq.~\eqref{eqn:reconstruction_cd}) generalizes well to EMD-based metrics than l-GAN.
% Although SetVAE is trained with CD (Eq.~\eqref{eqn:reconstruction_cd}), we note that it relatively generalizes well to EMD-based metrics than l-GAN.

Figure \ref{fig:compare_pointflow} illustrates qualitative comparisons.
%{\color{purple}Unlike PointFlow, we observe that SetVAE generates sharper details, including shapes of airplane wings/engines and car wheels. The sharper details are due to subset-level reasoning which is a meaningful gain from hierarchical latent variables. We analyze our model's powerful subset-level reasoning in \ref{sec:qualitative}.}
Compared to PointFlow, we observe that SetVAE generates sharper details, especially in small object parts such as wings/engines of an airplane or wheels of a car.
We conjecture that this is because our model generates samples considering inter-element dependency while capturing shapes in various granularities via hierarchical latent structure. 
% We conjecture that the higher fidelity is obtained from SetVAE's \jw{hierarchical model framework}, which allows it to choose an adequate level or resolution to model a fine-grained part.} % hierarchical subset reasoning

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/fig-5-cardinality.pdf}
    \vspace{-0.2cm}
    \caption{
    Samples from SetVAE for different cardinalities. At each row, the hierarchical latent variables are fixed and the initial set is re-sampled with different cardinality. 
    % \shcmt{Remove the boundary of small figures.}
    % \shcmt{add one row of comparison to PointFlow.}
    }
    \label{fig:cardinality}
    \vspace{-0.5cm}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/mega-cardinality.pdf}
    \caption{
    Samples from SetVAE and PointFlow in a high cardinality setting. Only the initial sets are re-sampled.
    }
    \label{fig:mega-cardinality}
    \vspace{-0.5cm}
\end{figure}

\subsection{Internal Analysis}
\label{sec:qualitative}
% In this section, we provide a qualitative analysis of SetVAE.
% We first show that SetVAE disentangles the global identity from a set's cardinality and generalizes very well to unseen cardinality.
% Then, we visualize the attention of SetVAE by color-coding the input/output and show that SetVAE learns semantically meaningful subset relations that are invariant to cardinality.
% We then provide an analysis of the hierarchical representations learned by SetVAE, demonstrating the coarse-to-fine composition of the latent features.
% Finally, we perform an ablation study to provide a better understanding of the components of SetVAE.

% \cutparagraphup
% \paragraph{Cardinality disentanglement and generalization}
\paragraph{Cardinality disentanglement}
% SetVAE can disentangle the cardinality of a set from the rest of generative factors (\emph{e.g.}, structure, style) in principle, as they are modeled independently by the initial set $\mathbf{z}^{(0)}$ and latent variables $\mathbf{z}^{(1:L)}$, respectively.
% To demonstrate this, we generate samples by changing the cardinality of the initial set while fixing the rest.
% Figure~\ref{fig:cardinality} illustrates the result.
% Ideally, SetVAE should be able to disentangle the cardinality of a set from the rest of generative factors (\emph{e.g.}, structure, style). 
Ideally, a generative model for sets should be able to disentangle the cardinality of a set from the rest of the generative factors (\emph{e.g.}, structure, style). 
SetVAE partly achieves this by decomposing the latent variables into the initial set $\mathbf{z}^{(0)}$ and the hierarchical latent variables $\mathbf{z}^{(1:L)}$.
% ... changing the cardinality of the initial set ...
To validate this, we generate samples by changing the initial set's cardinality while fixing the rest.
Figure~\ref{fig:cardinality} illustrates the result.
% To investigate how cardinality affects generation, we generated samples with initial sets with different sizes while fixing the hierarchical latent variables.
We observe that SetVAE generates samples having consistent global structure with a varying number of elements.
%showing that it reasonably disentangles the cardinality from the rest of factors characterizing an object. 
% More surprisingly ...
Surprisingly, it even generalizes well to the cardinalities not seen during training.
% ... maximum of 250 points ...
For instance, the model generalizes to any cardinality between 100 and 10,000, although it is trained with only 2048 points in ShapeNet and less than 250 points in Set-MNIST.
% In ShapeNet, we observe that the model generalizes to any cardinality between 100-10000, although it is trained with 2048 points only.
% We observe similar behavior in MNISTs, where the model generalizes to more than 40 times bigger set than the maximum cardinality of training data.
It shows that SetVAE disentangles the cardinality from the factors characterizing an object.

We compare SetVAE to PointFlow in extremely high cardinality setting (100k points) in Figure~\ref{fig:mega-cardinality}.
Although PointFlow innately disentangles cardinality by modeling each element independently, we observe that it tends to generate noisy, blurry boundaries in large cardinality settings.
In contrast, SetVAE retains the sharpness of the structure even for extreme cardinality, presumably because it considers inter-element dependency in the generation process.
% {\color{red}we find that out-of-distribution elements of the initial set translates to blurry output in a high cardinality setting.}
% In contrast, by modeling element dependency via subset representations, {\color{red}SetVAE can suppress outlier elements} and retain the shape's sharpness even when the cardinality reaches 100,000.

% {\color{red}
% Surprisingly, in all datasets, we observe that SetVAE always generates a consistent global set structure, disentangling it from cardinality.
% To further test SetVAE's cardinality generalization, we generated samples with unseen cardinality and observed that SetVAE generalizes very well to arbitrary cardinality without degradation of shape.
% In Set-MNIST, the model generalizes to up to {\color{red}40} times the maximum cardinality seen during training.
% In ShapeNet, we even observe that the model generalizes to any cardinality between {\color{red}100-10000}, although only 2048-sized sets were used for training.} {\fontfamily{cmss}\selectfont\color{red}[We conjecture that this property comes from the latent bottleneck.]}

\paragraph{Discovering coarse-to-fine dependency} %Partitioned subset reasoning
The SetVAE discovers interesting subset structures via hierarchical bottlenecks in ISAB and ABL.
To demonstrate this, we visualize the encoder attention (Eq.~\eqref{eqn:isab_bottleneck}) and generator attention (Eq.~\eqref{eqn:abl_bottleneck}) in Figure~\ref{fig:subset}, where each point is color-coded based on its hard assignment to one of $m$ inducing points
\footnote{Due to the difficulties in visualizing attention with multiple heads, we present a result of single-head attention model for illustration purposes.}.
% \footnote{For illustration purpose, we visualize the result using a single-head attention model.}.
% We observe that SetVAE attends to semantically interesting parts consistently across samples, such as wings and engines of an airplane, and legs and backs of a chair.
We observe that SetVAE attends to semantically interesting parts consistently across samples, such as wings and engines of an airplane, legs and backs of a chair, and even different instances of multiple digits.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/fig-6.pdf}
    \caption{
    Attention visualization at a selected layer.
    Each point is color-coded by its assignment based on attention. %to the inducing points.
    % Color-coded point-wise attention.
    % We plot encoder the attention on the reconstruction target, and decoder attention on generated data. 
    %\shcmt{Revise visualization and make parts more visible (especially Airplane)}
    %\shcmt{Remove the example in MultiMNIST such that it shows better disentanglement of digits.}
    %\shcmt{Make color coding in Generator fixed.}
    % \shcmt{Change it to single column.}
    }
    \label{fig:subset}
    \vspace{-0.3cm}
\end{figure}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/fig-7.pdf}
    \caption{Visualization of encoder attention across multiple layers.
    IP notes the number of inducing points at each level.
    See the supplementary file for more results.
    % More examples can be found in Section~\ref{appendix:suppresults} of the supplementary file.
    %\shcmt{Add a figure of hierarchical composition. Two layer would be enough.}
    }
    \label{fig:composition}
    \vspace{-0.4cm}
\end{figure}

Figure~\ref{fig:composition} illustrates the point-wise attention across levels.
% At a coarse level, the encoder decomposes an object into two disjoint parts, while they are defined in much finer granularity in the subsequent levels.
We observe that the top-level tends to capture the coarse and symmetric structures, such as wings and wheels, which are further decomposed into much finer granularity in the subsequent levels.
We conjecture that this coarse-to-fine subset dependency helps the model to generate accurate structure in various granularity from global structure to local details. 
% As we discussed earlier, this helps the model to generate accurate structure in various granularity from global shape to local details. 
% In the finer levels, each objects are decomposed into the finer granularity.

% \jw{Here, the encoder decomposes an object to two disjoint parts, describing input's features in a coarse-level.
% In the fine level, we observe that these coarse parts are distributed further into fine-grained subsets.
% This implies that subset information is implicitly passed across hierarchies, imposing a subset dependency over multiple levels and scales.}
%It shows that interesting subset dependencies are implicitly captured by our method, and imposed 
%For instance, {\color{blue} add discussion}.

% ... leads to an interesting disentanglement ...
Interestingly, we find that hierarchical structure of SetVAE sometimes leads to a disentanglement of generative factors across layers.
% We investigate the role of the latents by learning two classifiers on top of each latent 
% To demonstrate this, we train two classifiers in Set-MultiMNIST to recognize digit identity and position using each latent variable $\mathbf{z}^{(l)}$ as an input. 
To demonstrate this, we train two classifiers in Set-MultiMNIST, one for digit class and the other for their positions.
% ... each layer of the SetVAE encoder as an input ...
We train the classifiers using latent variable at each layer of the generator as an input, and measure the accuracy at each layer.
In Figure~\ref{fig:lda}, the latent variables at the lower layers tend to contribute more in locating the digits, while higher layers contribute in generating shape.
% We validate the role of each latent set by analyzing the learned latent space group-by-group in MultiMNIST.
% We perform LDA for each latent set. One predicts binned location of digits, and another predicts identity of the digits.
% In Figure \ref{fig:lda}, we show that low-res, upper latent sets encodes coarse digit positions, and a high-res, lower latent sets encode fine digit identities.

%{\color{purple}This property adopts SetVAE to perform well with a few parameters.}
%In Figure \ref{fig:subset-cardinality}, we demonstrate that the encoder/decoder attention is indeed invariant to cardinality of the input set.
\iffalse
This subset-wise reasoning offers essential advantages.
Subset reasoning allows SetVAE to effectively reduce the number of parameters by amortizing elementwise reasoning cost.
We also observe that each subset representation is invariant to the input set's cardinality, {\color{red}and suppose that subset reasoning may support SetVAE's generalization to different cardinality. \color{red}Need more Explanation.}
The observation is demonstrated in Figure \ref{fig:subset-cardinality}.
\fi

\begin{figure}[!t]
\centering
    \includegraphics[width=0.55\linewidth]{figures/lda.pdf}
    \vspace{-0.3cm}
    \caption{
    Layer-wise classification results using the hierarchical latent variables in Set-MultiMNIST dataset. 
    % Latent at the first layer contributes most in locating the digit, while the one at third layer contribute more in shaping it.
    % The performance of auxiliary networks in inferring data composition of each hierarchy. 
    % Low-res, upper latent sets encode coarse digit positions, and high-res, lower latent sets encode fine digit identities.
    }
    \label{fig:lda}
    \vspace{-0.2cm}
\end{figure}

\iffalse
\paragraph{Multi-level}
% \begin{figure}[!t]
%     \centering
%     % \includegraphics{}
%     \vspace{3cm}
%     [Figure] Hierarchical mixing in ShapeNet Airplane, MNIST, and MultiMNIST {\color{red}(Progressive mixing as in NVAE? like now as in StyleGAN?)}
%     \vspace{3cm}
%     \caption{Two sets of latent variables were inferred from respective data (sources A and B). The rest of the sets were generated by replacing a specific latent set of source A at a certain hierarchy to corresponding latent set in source B.}
%     \label{fig:mix}
% \end{figure}

SetVAE learns coarse-to-fine subset relations via multi-scale hierarchical latent sets.
By setting the top-down hierarchical latent set scales to increase gradually, we observe that the model learns a coarse-to-fine composition of data.
% ... another data ...
We demonstrate this by replacing a latent set at a specific hierarchy with a latent set from \jw{other} data and observing modified visual features. The qualitative results are demonstrated in Figure \ref{fig:mix}.

\jw{We further assess the learned hierarchical latent sets in Set-MultiMNIST, where coarse-to-fine composition (e.g. location to digit identities) is evident.}
We validate the role of each latent set by analyzing the learned latent space group-by-group in Set-MultiMNIST.
We perform LDA for each latent set. One predicts binned location of digits, and another predicts identity of the digits.
In Figure \ref{fig:lda}, we show that low-res, upper latent sets encodes coarse digit positions, and a high-res, lower latent sets encode fine digit identities.
\fi

%\cutparagraphup
% \subsection{Ablation Study}
\cutparagraphup
\paragraph{Ablation study}  
% To better understand the contribution of each components of SetVAE, we conduct an ablation study on Set-MultiMNIST.
Table~\ref{table:ablation} summarizes the ablation study of SetVAE (see the supplementary file for qualitative results and evaluation detail).
We consider two baselines for comparison: Vanilla SetVAE employing a global latent variable $\mathbf{z}^{(1)}$ (Section~\ref{sec:method}), and hierarchical SetVAE with unimodal prior (Section~\ref{sec:implementation}).
% Table~\ref{table:ablation} summarizes the result (See the supplementary file for qualitative results).

The Vanilla SetVAE performs much worse than our full model.
% We conjecture that it is because ...
We conjecture that a single latent variable is not expressive enough to encode complex variations in MultiMNIST, such as identity and position of multiple digits.
% On the other hand, exploiting rich hierarchical latent structure allows our full model to decompose these factors much more easily.
We also find that multi-modal prior stabilizes the training of attention and guides the model to better local optima.
% We conjecture that multiple modes can guide the inducing points to bind to each of them during initial stages of training, speeding up the learning process of attention.
% For comparison, we implement Vanilla SetVAE in Section~\ref{sec:formulation} using the same bidirectional network but by pooling 
% The results are summarized in Figure \ref{fig:ablation} and Table \ref{table:ablation}. We provide supplementary results in Section~\ref{appendix:ablation} of appendix.

% \cutparagraphup
% \paragraph{Hierarchy:}  
% We make a non-hierarchical, basic SetVAE by pooling all induced set elements from bottom-up encoder to predict a single latent element, and using it as $\mathbf{z}$ in all decoder ABLs.
% We observe that hierarchical subset reasoning is critical for modeling compositional data.

% \cutparagraphup
% \paragraph{Initial set:} 
% We remove the multiple modes in the initial set distribution by using only one component (plain Gaussian).
% We observe that the multimodal initial set is essential to training stabilization once there are a number of data modes.

\begin{table}[t!]
\begin{center}
\caption{Ablation study performed on Set-MultiMNIST dataset using FID scores for {$64\times 64$} rendered images.}
\vspace{-0.2cm}
\footnotesize
\label{table:ablation}
\begin{tabular}{lc}
\Xhline{2\arrayrulewidth}
\\[-1em] Model & FID($\downarrow$) \\
\\[-1em]\Xhline{2\arrayrulewidth}
\\[-1em]
SetVAE & 1062 \\
Non-hierarchical & 1470 \\
Unimodal prior & 1252 \\
\\[-1em]\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\vspace{-0.6cm}
\end{table}

==> cvpr_draft/introduction.tex <==
% !TEX root = cvpr.tex
\section{Introduction}
\label{sec:intro}
\ifdefined\paratitle {\color{blue}
[There has been an increasing demand on ML for set data: give some examples of set data] \\
} \fi
There have been increasing demands in machine learning for handling \emph{set-structured} data (\emph{i.e.}, a group of unordered instances).
Examples of set-structured data include object bounding boxes~\cite{li2019grains, carion2020endtoend}, point clouds~\cite{achlioptas2018learning, li2018point}, support sets in the meta-learning~\cite{finn2017modelagnostic}, \emph{etc.}
While initial research mainly focused on building neural network architectures to encode sets~\cite{zaheer2017deep,lee2019set}, generative models for sets have recently grown popular~\cite{zhang2020deep,kosiorek2020conditional, stelzner2020generative,yang2019pointflow, yang2020energybased}.
%, where the goal is to build a model to generate set-structured data.
% While recent efforts have been mostly focused on encoding of the set data, unsupervised generative modeling of sets has been relatively less explored~\cite{zhang2020deep,kosiorek2020conditional, stelzner2020generative,yang2019pointflow, yang2020energybased}.

\ifdefined\paratitle {\color{blue}
[In this paper, we explore a generative model for set: introduce some recent works in set generation. Discuss what poses the unique challenges in set generative modeling. ] \\
} \fi
A generative model for set-structured data should verify the two essential requirements: (i) \textit{exchangeability}, meaning that a probability of a set instance is invariant to its elements' ordering, and (ii) handling \textit{variable cardinality}, meaning that a model should flexibly process sets with variable cardinalities.
These requirements pose a unique challenge in set generative modeling, as they prevent the adaptation of standard generative models for sequences or images~\cite{goodfellow2014generative, karras2019stylebased, oord2016pixel,oord2016conditional}. 
For instance, typical operations in these models, such as convolution or recurrent operations, exploit implicit ordering of elements (\emph{e.g.}, adjacency), thus breaking the exchangeability.
Several works circumvented this issue by imposing heuristic ordering~\cite{hong2018inferring, eslami2016attend, greff2019multi, ritchie2019fast}.
% For instance, \cite{hong2018inferring} proposes a generative model for sequences with variable sizes but assumes orderings for the sequences and thus breaks the exchangeability. 
%When applied to set-structured data, however, any ordering assumed by a model act as an unnecessary inductive bias that might harm the generalization ability.
However, when applied to set-structured data, any ordering assumed by a model imposes an unnecessary inductive bias that might harm the generalization ability.

\begin{figure}[t]
\begin{center}
    \includegraphics[width=0.47\textwidth]{figures/fig-1-ann-1.pdf}
    %\vspace{-0.22in}
\end{center}
    \caption{Color-coded attention learned by SetVAE encoder for three data instances of ShapeNet Airplane \cite{chang2015shapenet}. Level 1 shows attention in the most coarse scale. Level 2 and 3 show attention in more fine-scales.
    %\shcmt{No clue to understand this figure.}
    }
\label{fig:eyecatcher}
\end{figure}

\begin{table*}[!ht]
\centering
\footnotesize
%Summary of several set generative frameworks available to date. Our SetVAE jointly achieves desirable properties, with the advantages of VAE framework combined with our novel contributions.
\caption{Summary of several set generative frameworks available to date. Our SetVAE jointly achieves desirable properties, with the advantages of VAE framework combined with our novel contributions.
}
\begin{tabular}{l>{\centering}m{0.12\textwidth}>{\centering}m{0.1\textwidth}>{\centering}m{0.12\textwidth}>{\centering\arraybackslash}m{0.1\textwidth}}
\Xhline{2\arrayrulewidth}
\\[-1em] Model & Exchangeability & \shortstack{Variable\\cardinality} & \shortstack{Inter-element\\dependency} & \shortstack{Hierachical\\latent structure} \\
\\[-1em]\Xhline{2\arrayrulewidth}
\\[-1em]
l-GAN \cite{achlioptas2018learning} & $\times$ & $\times$ & $\bigcirc$ & $\times$ \\
PC-GAN \cite{li2018point} & $\bigcirc$ & $\bigcirc$ & $\times$ & $\times$ \\
PointFlow \cite{yang2019pointflow} & $\bigcirc$ & $\bigcirc$ & $\times$ & $\times$ \\
% GAST \cite{stelzner2020generative} & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\times$ \\
EBP \cite{yang2020energybased} & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\times$ \\
\\[-1em]\hline
\\[-1em] SetVAE (ours) & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ \\
\\[-1em]\Xhline{2\arrayrulewidth}
\end{tabular}
\label{table:framework}
\end{table*}

\ifdefined\paratitle {\color{blue}
[However, existing models for set has several limitations: discuss their limitations, and argue that our model handles them] \\
} \fi
There are several existing works satisfying these requirements.
%... while other approaches are built upon various generative models,
Edwards et al.,~\cite{edwards2017neural} proposed a simple generative model encoding sets into latent variables, while other approaches build upon various generative models, such as generative adversarial networks~\cite{li2018point, stelzner2020generative}, flow-based models~\cite{yang2019pointflow,kim2020softflow}, and energy-based models~\cite{yang2020energybased}. 
% \cite{li2018point, stelzner2020generative} proposed generative adversarial networks for sets. \cite{yang2019pointflow,kim2020softflow} proposed flow-based models for sets, and \cite{yang2020energybased} introduced energy-based model for sets. 
All these works define valid generative models for set-structured data, but with some limitations.
% \cite{edwards2017neural,li2018point, yang2019pointflow} process elements in sets independently, so the models cannot effectively reflect the interactions between the elements during the generation. \cite{stelzner2020generative, yang2020energybased} take the inter-element dependency into account, but \cite{stelzner2020generative} sets an upper bound on the number of elements to generate, and \cite{yang2020energybased} is based on an energy-based model from which is costly to generate samples.
% To achieve exchangeability, many approaches process elements in sets independently, limiting the models to unable to reflect the interactions between the elements during the generation.
To achieve exchangeability, many approaches process set elements independently~\cite{li2018point, yang2019pointflow}, limiting the models in reflecting the interactions between the elements during generation.
% ... but has an upper bound
Some approaches take the inter-element dependency into account~\cite{stelzner2020generative, yang2020energybased}, but have an upper bound on the number of elements~\cite{stelzner2020generative}, or less scalable due to heavy computations~\cite{yang2020energybased}.
% assume independence between elements in sets  given a global latent variable, which could ignore interactions between set elements and limit the model's flexibility.
% Some models take inter-element dependency into account \cite{stelzner2020generative, yang2020energybased}, but \cite{stelzner2020generative} poses an upper bound on the number of elements to generate, and \cite{yang2020energybased} is based on an energy-based model from which is costly to generate samples.
% More importantly, the existing models ... via a single-level representation.
More importantly, existing models are less effective in capturing subset structures in sets presumably because they represent a set with a single-level representation.
% ... much beneficial ...
For sets containing multiple sub-objects or parts, it would be beneficial to allow a model to have structured latent representations such as one obtained via hierarchical latent variables.
% Imagine a set containing multiple sub-objects or decomposed into multiple parts. 
% For such data, it would be beneficial to allow a model to have structured latent representations such as one obtained via hierarchical latent variables.

% More importantly, current approaches are limited in representing complex subset interactions existing within a set instance, which are imposed by multiple object instances, composition of parts within an object, \etc.
% To capture such structures efficiently, we argue that a generative framework should allows more expressible latent structures.}

\ifdefined\paratitle {\color{blue}
[We propose a hierarchical Variational Autoencoder for set: give an overview of our method. discuss how it addresses the limitations in the existing methods] \\
} \fi
In this paper, we propose SetVAE, a novel hierarchical variational autoencoder (VAE) for sets. SetVAE models interaction between set elements by adopting attention-based Set Transformers \cite{lee2019set} into the VAE framework, and extends it to a \textit{hierarchy} of latent variables \cite{sonderby2016ladder, vahdat2020nvae} to account for flexible subset structures.
By organizing latent variables at each level as a \textit{latent set} of fixed cardinality, SetVAE is able to learn hierarchical multi-scale features that decompose a set data in a coarse-to-fine manner (Figure \ref{fig:eyecatcher}) while achieving \textit{exchangeability} and handling \textit{variable cardinality}.
In addition, composing latent variables invariant to input's cardinality allows our model to generalize to arbitrary cardinality unseen during training.

\ifdefined\paratitle {\color{blue}
[Discuss the contribution of our work using the bullet-items.] \\
} \fi
The contributions of this paper are as follows:
\begin{itemize}
    \item We propose SetVAE, a novel hierarchical VAE for sets with \textit{exchangeability} and \textit{varying cardinality}.  To the best of our knowledge, SetVAE is the first VAE successfully applied for sets with arbitrary cardinality. SetVAE has a number of desirable properties compared to previous works, as summarized in Table \ref{table:framework}.
    \item Equipped with novel Attentive Bottleneck Layers (ABL), SetVAE is able to model the coarse-to-fine dependency across the arbitrary number of set elements using a hierarchy of latent variables.
    \item We conduct quantitative and qualitative evaluations of SetVAE on generative modeling of point cloud in various datasets, and demonstrate better or competitive performance in generation quality with less number of parameters than the previous works.
\end{itemize}

%\jw{The rest of this paper is organized as follows. After providing a background for set generation and encoding in Section \ref{sec:preliminary}, we introduce the SetVAE in Section \ref{sec:method} and \ref{sec:architecture}. We present relations to previous works in Section \ref{sec:related}, and discuss experimental results in ShapeNet \cite{chang2015shapenet}, Set-MNIST \cite{zhang2020deep}, and Set-MultiMNIST \cite{eslami2016attend} in Section \ref{sec:experiment}.}


==> cvpr_draft/method.tex <==
% !TEX root = cvpr.tex
\section{Variational Autoencoders for Sets}
\label{sec:method}
% We now introduce a SetVAE, a Variational Autoencoder for sets that exploits the hierarchical latent structure while retaining \textit{exchangeability} and can incorporate \textit{variable cardinality}.
% We first describe its formulation and introduce the architecture that satisfies the exchangeability.
% In this section, we derive a VAE objective for handling set-structured data, where its architecture is introduced in the next section.
% As we discussed earlier, VAE for set should be able to handle the arbitrary cardinality while satisfying the exchangeability of the likelihood.
The previous section suggests that there are two essential requirements for VAE for set-structured data: it should be able to model the likelihood of sets (i) in arbitrary cardinality, and (ii) invariant to the permutation (\emph{i.e.,} exchangeable). 
% This section introduces our VAE objective for set of arbitrary size, while modeling the exchangeable likelihood is discussed in Section~\ref{sec:architecture}.
This section introduces our SetVAE objective that satisfies the first requirement, while achieving the second requirement is discussed in Section~\ref{sec:architecture}.

The objective of VAE \cite{kingma2014autoencoding} is to learn a generative model $p_\theta(\mathbf{x}, \mathbf{z}) = p_\theta(\mathbf{z}) p_\theta(\mathbf{x}|\mathbf{z})$ for data $\mathbf{x}$ and latent variables $\mathbf{z}$. 
Since the true posterior is unknown, we approximate it using the inference model $q_\phi(\mathbf{z}|\mathbf{x})$ and optimize the variational lower bound (ELBO) of the marginal likelihood $p(\mathbf{x})$:
% VAE \cite{kingma2014autoencoding} trains a generative model $p_\theta(\mathbf{x}, \mathbf{z}) = p_\theta(\mathbf{z}) p_\theta(\mathbf{x}|\mathbf{z})$ for data $\mathbf{x}$ and latent variables $\mathbf{z}$, with an inference model $q_\phi(\mathbf{z}|\mathbf{x})$ that approximates true posterior by optimizing a variational lower bound (ELBO) of the likelihood $p(\mathbf{x})$:
%
\begin{equation}
    % \log p(\mathbf{x})\geq \mathbb{E}_{q_\phi(\mathbf{z}|\mathbf{x})}{\left[\log p_\theta(\mathbf{x}|\mathbf{z})\right]}  - D_{KL}\left(q_\phi(\mathbf{z}|\mathbf{x})||p_\theta(\mathbf{z})\right)
    \mathcal{L}_{\text{VAE}} = \mathbb{E}_{q_\phi(\mathbf{z}|\mathbf{x})}{\left[\log p_\theta(\mathbf{x}|\mathbf{z})\right]}  - \text{KL}\left(q_\phi(\mathbf{z}|\mathbf{x})||p_\theta(\mathbf{z})\right).
    \label{eqn:original_vae}
\end{equation}

\cutparagraphup
\paragraph{Vanilla SetVAE}
% A VAE for set should treat $\mathbf{x}$ as a set of $n$ elements, $\mathbf{x}=\{\mathbf{x}_i\}_{i=1}^n$.
% The problem is how to enable an arbitrary cardinality $n$.
When our data is a set $\mathbf{x}=\{\mathbf{x}_i\}_{i=1}^n$, Eq.~\eqref{eqn:original_vae} should be modified such that it can incorporate the set of arbitrary cardinality $n$\footnote{Without loss of generality, we use $n$ to denote the cardinality of a set but assume that the training data is composed of sets in various size.}.
To this end, we propose to decompose the latent variable $\mathbf{z}$ into the two independent variables as $\mathbf{z}=\{\mathbf{z}^{(0)}, \mathbf{z}^{(1)}\}$.
We define $\mathbf{z}^{(0)}=\{\mathbf{z}_i^{(0)}\}_{i=1}^n$ to be a set of \textit{initial elements}, whose cardinality is always the same as a data $\mathbf{x}$. 
Then we model the generative process as transforming $\mathbf{z}^{(0)}$ into a set $\mathbf{x}$ conditioned on the $\mathbf{z}^{(1)}$.

% We assume $\mathbf{z}^{(0)}\perp\mathbf{z}^{(1)}$, so that the prior $p(\mathbf{z})$ is equal to $p(\mathbf{z}^{(0)})p(\mathbf{z}^{(1)})$.
% We assume $\mathbf{z}^{(0)}\perp\mathbf{z}^{(1)}$ such that $p(\mathbf{z})=p(\mathbf{z}^{(0)})p(\mathbf{z}^{(1)})$.
Given the independence assumption, the prior is factorized by $p(\mathbf{z})=p(\mathbf{z}^{(0)})p(\mathbf{z}^{(1)})$.
The prior on initial set $p(\mathbf{z}^{(0)})$ is further decomposed into the cardinality and element-wise distributions as:
% To allow sampling $\mathbf{z}^{(0)}$ of arbitrary cardinality, we decompose $p(\mathbf{z}^{(0)})$ into the cardinality and element-wise distributions as:
%
\begin{equation}
    p(\mathbf{z}^{(0)}) = p(n)\prod_{i=1}^np(\mathbf{z}_{i}^{(0)}).
    \label{eqn:prior_initialset}
\end{equation}
%
% {\color{magenta} this is not clear; what is the empirical distribution? you mean $\delta_n$?}
% {\color{blue} We compute this by empirically counting the histogram of training set cardinality} 
We model $p(n)$ using the empirical distribution of the training data cardinality.
We find that the choice of the prior $p(\mathbf{z}_i^{(0)})$ is critical to the performance, and discuss its implementation in Section~\ref{sec:implementation}.

% To infer $\mathbf{z}^{(0)}$ and $\mathbf{z}^{(1)}$ given a data $\mathbf{x}$, we introduce approximate posterior $q(\mathbf{z}|\mathbf{x}) = q(\mathbf{z}^{(0)}|\mathbf{x})q(\mathbf{z}^{(1)}|\mathbf{x})$. Similar to Eq.~\eqref{eqn:prior_initialset}, $q(\mathbf{z}^{(0)}|\mathbf{x})$ can be further decomposed as:
Similar to the prior, the approximate posterior is defined as $q(\mathbf{z}|\mathbf{x}) = q(\mathbf{z}^{(0)}|\mathbf{x})q(\mathbf{z}^{(1)}|\mathbf{x})$ and decomposed into:
\begin{equation}
    q(\mathbf{z}^{(0)}|\mathbf{x}) = q(n|\mathbf{x})\prod_{i=1}^nq(\mathbf{z}_{i}^{(0)}|\mathbf{x})
    \label{eqn:posterior_vanillaSetVAE}
\end{equation}
%
We define $q(n|\mathbf{x})=\delta(n)$ as a delta function with $n=|\mathbf{x}|$, and set $q(\mathbf{z}_{i}^{(0)}|\mathbf{x}) = p(\mathbf{z}_{i}^{(0)})$ similar to \cite{yang2019pointflow, kosiorek2020conditional, locatello2020objectcentric}.
% To simplify training, we fix $q(\mathbf{z}_{i}^{(0)}|\mathbf{x}) = p(\mathbf{z}_{i}^{(0)})$, and let $q(n|\mathbf{x})=\delta(n)$ which is an indicator function with value $1$ only if $n=|\mathbf{x}|$, else $0$. In other words, we sample $\mathbf{z}^{(0)}$ with same cardinality to $\mathbf{x}$ during its reconstruction.
The resulting ELBO can be written as
%
\begin{align}
    \mathcal{L}_{\text{SVAE}}&= \mathbb{E}_{q(\mathbf{z}|\mathbf{x})}{\left[ \log p(\mathbf{x}|\mathbf{z}) \right]} \nonumber\\
    &- \textnormal{KL}(q(\mathbf{z}^{(0)}|\mathbf{x})||p(\mathbf{z}^{(0)})) \nonumber\\
    &- \textnormal{KL}(q(\mathbf{z}^{(1)}|\mathbf{x})||p(\mathbf{z}^{(1)})).
    \label{eqn:elbo_vanillaSetVAE}
\end{align}
%
In the supplementary file, we show that the first KL divergence in Eq.~\eqref{eqn:elbo_vanillaSetVAE} is a constant and can be ignored in the optimization.
During inference, we sample $\mathbf{z}^{(0)}$ by first sampling the cardinality $n\sim p(n)$ then the $n$ initial elements independently from the prior $p(\mathbf{z}_{i}^{(0)})$.
%{\color{blue} we may need to discuss the sampling of $\mathbf{z}^{(1)}$}.
% {\color{OliveGreen}Unlike $\mathbf{z}^{(0)}$, $\mathbf{z}^{(1)}$ can be regarded a plain latent variable, \eg with tractable prior $p(\mathbf{z}^{(1)}) = \mathcal{N}(0, \mathbf{1})$ and approximate posterior $q(\mathbf{z}^{(1)}|\mathbf{x}) = \mathcal{N}(\mu, \sigma)$. 
% In Section~\ref{sec:architecture}, we discuss how $\mu, \sigma$ can be inferred from $\mathbf{x}$, and how $\mathbf{z}^{(1)}$ can condition the transformation of $\mathbf{z}^{(0)}$ to $\mathbf{x}$.}

\cutparagraphup
\paragraph{Hierarchical SetVAE}
% Unlike the initial set $\mathbf{z}^{(0)}$ in the above formulation, $\mathbf{z}^{(1)}$ can be regarded a plain latent variable, \eg with tractable prior $p(\mathbf{z}^{(1)}) = \mathcal{N}(0, \mathbf{1})$ and approximate posterior $q(\mathbf{z}^{(1)}|\mathbf{x}) = \mathcal{N}(\mu, \sigma)$. 
To allow our model to learn a more expressive latent structure of the data, we can extend the vanilla SetVAE using hierarchical latent variables. 
% Among the two terms, we choose to keep $p(\mathbf{z}^{(0)})$ minimal and make $p(\mathbf{z}^{(1)})$ more flexible by extending $\mathbf{z}^{(1)}$ into $L$ disjoint groups $\{\mathbf{z}^{(1)}, ..., \mathbf{z}^{(L)}\}$ and introducing a hierarchical dependency across them.

% Specifically, for $\{\mathbf{z}^{(1)}, ..., \mathbf{z}^{(L)}\}$, we introduce a top-down dependency that for every $l>1$, $\mathbf{z}^{(l)}$ depends on $\{\mathbf{z}^{(0)}, ..., \mathbf{z}^{(l-1)}\}$.
% ... the $L$ disjoint groups
Specifically, we extend the plain latent variable $\mathbf{z}^{(1)}$ into $L$ disjoint groups $\{\mathbf{z}^{(1)}, ..., \mathbf{z}^{(L)}\}$, and introduce a top-down hierarchical dependency between $\mathbf{z}^{(l)}$ and $\{\mathbf{z}^{(0)}, ..., \mathbf{z}^{(l-1)}\}$ for every $l>1$. 
This leads to the modification in the prior and approximate posterior to
\begin{align}
    p(\mathbf{z}) &= p(\mathbf{z}^{(0)}) p(\mathbf{z}^{(1)}) \prod_{l>1} {p(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)})}\label{eqn:prior}\\
    q(\mathbf{z}|\mathbf{x}) &= q(\mathbf{z}^{(0)}|\mathbf{x}) q(\mathbf{z}^{(1)}|\mathbf{x}) \prod_{l>1} {q(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)}, \mathbf{x})}. \label{eqn:posterior}
\end{align}
% To infer $\{\mathbf{z}^{(1)}, ..., \mathbf{z}^{(L)}\}$ given $\mathbf{x}$, we keep the top-down dependency order and write the approximate posterior as follows:
% %
% \begin{align}\label{posterior}
%     q(\mathbf{z}|\mathbf{x}) &= q(\mathbf{z}^{(0)}|\mathbf{x}) q(\mathbf{z}^{(1)}|\mathbf{x}) \prod_{l>1} {q(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)}, \mathbf{x})}
% \end{align}

% We now derive the ELBO of the hierarchical VAE, extended from Equation \ref{elbo_set} as follows:
Applying Eq.~\eqref{eqn:prior} and \eqref{eqn:posterior} to Eq.~\eqref{eqn:elbo_vanillaSetVAE}, we can derive the ELBO as
\begin{align}
    &\mathcal{L}_{\text{HSVAE}} = \mathbb{E}_{q(\mathbf{z}|\mathbf{x})}{\left[ \log p(\mathbf{x}|\mathbf{z}) \right]} \nonumber\\
    &~~- \textnormal{KL}(q(\mathbf{z}^{(0)}|\mathbf{x})||p(\mathbf{z}^{(0)})) - \textnormal{KL}(q(\mathbf{z}^{(1)}|\mathbf{x})||p(\mathbf{z}^{(1)})) \nonumber\\
    &~- \sum_{l=2}^L{\mathbb{E}_{q(\mathbf{z}^{(<l)}|\mathbf{x})}{\textnormal{KL}(q(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)}, \mathbf{x})||p(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)})}}.
    % &\mathcal{L}_{\text{HSVAE}} = \mathbb{E}_{q(\mathbf{z}|\mathbf{x})}{\left[ \log p(\mathbf{x}|\mathbf{z}) \right]} - \textnormal{KL}(q(\mathbf{z}^{(1)}|\mathbf{x})||p(\mathbf{z}^{(1)})) \nonumber\\
    % &~- \sum_{l=2}^L{\mathbb{E}_{q(\mathbf{z}^{(<l)}|\mathbf{x})}{\textnormal{KL}(q(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)}, \mathbf{x})||p(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)})}}.
    \label{eqn:elbo_hierarchicalSetVAE}
\end{align}
% The expectation $\mathbb{E}_{q(\mathbf{z}^{(<l)}|\mathbf{x})}[\cdot]$ can be approximated with 1-sample Monte Carlo estimation from the approximate posterior $q(\mathbf{z}^{(<l)}|\mathbf{x}) = q(\mathbf{z}^{(0)}|\mathbf{x}) q(\mathbf{z}^{(1)}|\mathbf{x}) \prod_{i=2}^{l-1} {q(\mathbf{z}^{(i)}|\mathbf{z}^{(<i)}, \mathbf{x})}$.

\cutparagraphup
\paragraph{Hierarchical prior and posterior}
To model the prior and approximate posterior in Eq.~\eqref{eqn:prior} and \eqref{eqn:posterior} with top-down latent dependency, we employ the bidirectional inference in \cite{sonderby2016ladder}.
% We outline the formulations here, and elaborate the computations in Section~\ref{sec:architecture}.
We outline the formulations here and elaborate on the computations in Section~\ref{sec:architecture}. 

Each conditional $p(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)})$ in the prior is modeled by the factorized Gaussian, whose parameters are dependent on the latent variables of the upper hierarchy $\mathbf{z}^{(<l)}$:
%In VAE, the priors and approximate posteriors are often parameterized as simple tractable distribution such as factorial Gaussian. Following the convention, we parameterize each conditional of the prior $p(\mathbf{z})$ in Eq.~\eqref{eqn:prior} as:
\begin{equation}
    p(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)}) = \mathcal{N}\left(\mu_l(\mathbf{z}^{(<l)}), \sigma_l(\mathbf{z}^{(<l)})\right).
    \label{eqn:normal_prior}
\end{equation}
%As a special case, the top prior $p(\mathbf{z}^{(1)})$ has no dependency to $\mathbf{z}^{(0)}$, so we let $p(\mathbf{z}^{(1)}) = \mathcal{N}(\mu_1, \sigma_1)$.

Similarly, each conditional in the approximate posterior $q(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)}, \mathbf{x})$ is also modeled by the factorized Gaussian.
We use the residual parameterization in \cite{vahdat2020nvae} which predicts the parameters of the Gaussian using the displacement and scaling factors ($\Delta\mu$,$\Delta\sigma$) conditioned on $\mathbf{z}^{(<l)}$ and $\mathbf{x}$:
%For the approximate posterior $q(\mathbf{z}|\mathbf{x})$,
% {\color{OliveGreen}For each conditional $q(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)}, \mathbf{x})$ in the approximate posterior, previous works showed that using $\mathbf{x}$ to obtain a corrected version of the prior $p(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)})$ is beneficial to stabilizing VAE training.
% Adopting the residual parameterization \cite{vahdat2020nvae}, we correct the prior Gaussian distribution in Equation \ref{eqn:normal_prior} by applying displacement $\Delta\mu$ and scaling $\Delta\sigma$ predicted from $\mathbf{z}^{(<l)}$ and $\mathbf{x}$:}
\begin{align}
    q(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)}, \mathbf{x}) = \mathcal{N}(&\mu_l(\mathbf{z}^{(<l)}) + \Delta\mu_l(\mathbf{z}^{(<l)}, \mathbf{x}), \nonumber\\
    &\sigma_l(\mathbf{z}^{(<l)}) \cdot \Delta\sigma_l(\mathbf{z}^{(<l)}, \mathbf{x})).
    \label{eqn:normal_posterior}
\end{align}

% Note that the residual parameterization allows a cheap computation of the KL divergence \cite{vahdat2020nvae}:
% \begin{align}
%     \textnormal{KL}\left( \mathcal{N}(\mu + \Delta\mu, \sigma \cdot \Delta\sigma) || \mathcal{N}(\mu, \sigma) \right)\nonumber\\
%     = \frac{1}{2}\left( \frac{\Delta\mu^2}{\sigma^2} + \Delta\sigma^2 - \log\Delta\sigma^2 - 1 \right)
% \end{align}
\cutparagraphup
\paragraph{Invariance and equivariance}
\iffalse
{\color{magenta}
We are encoding a set $\mathbf{x}$ into an initial set $\mathbf{z}^{(0)}$ and latent variables $\mathbf{z}^{(1:L)}:=\{\mathbf{z}^{(l)}\}_{l=1}^L$.
Hence, it is natural to assume that $q(\mathbf{z}^{(0)}|\mathbf{x})$ is equivariant w.r.t. the permutation of $\mathbf{x}$ and
$q(\mathbf{z}^{(1:L)}|\mathbf{x})$ is invariant to the permutation of $\mathbf{x}$ (because we want a unique representation of $\mathbf{x}$).
Likewise, we assume that the decoding distribution $p(\mathbf{x}|\mathbf{z}^{(0)}, \mathbf{z}^{(1:L)})$ is equivariant to the permutation of $\mathbf{z}^{(0)}$.
}
\fi
We assume that the decoding distribution $p(\mathbf{x}|\mathbf{z}^{(0)}, \mathbf{z}^{(1:L)})$  is equivariant to the permutation of $\mathbf{z}^{(0)}$ and invariant to the permutation of $\mathbf{z}^{(1:L)}$ since such model induces an exchangeable model:
% If we assume that the encoding distributions $q(\mathbf{z}^{(0)}|\mathbf{x})$ and $q(\mathbf{z}^{(1:L)}|\mathbf{x})$ are invariant w.r.t. the permutation of $\mathbf{x}$, and the decoding distribution $p(\mathbf{x}|\mathbf{z}^{(0)}, \mathbf{z}^{(1:L)})$ is equivariant to the permutation of $\mathbf{z}^{(0)}$, 
% such decoder induces an exchangeable model since
\begin{align}
    \lefteqn{p(\pi(\mathbf{x})) = \int p(\pi(\mathbf{x})|\pi(\mathbf{z}^{(0)}), \mathbf{z}^{(1:L)}) p(\pi(\mathbf{z}^{(0)})) p(\mathbf{z}^{(1:L)}) d\mathbf{z}}\nonumber\\
    &= \int p(\mathbf{x}|\mathbf{z}^{(0)},\mathbf{z}^{(1:L)}) p(\mathbf{z}^{(0)}) p(\mathbf{z}^{(1:L)}) d\mathbf{z} = p(\mathbf{x}).
\end{align}
We further assume that $q(\mathbf{z}^{(0)}|\mathbf{x})$ is equivariant and $q(\mathbf{z}^{(1:L)}|\mathbf{x})$ is invariant to the permutation of $\mathbf{x}$.
% In the following section, we describe how we actually implement the encoder and decoder satisfying this criteria.
In the following section, we describe how we implement the encoder and decoder satisfying these criteria.

\section{SetVAE Framework}
\label{sec:architecture}
% In the Section~\ref{sec:method}, we formulated the prior, approximate posterior, and optimization objective of SetVAE.
% In this section, we develop an implementation of it based on Set Transformer \cite{lee2019set}.
We present the overall framework of the proposed SetVAE. 
Figure~\ref{fig:overview} illustrates an overview.
% Our VAE formulation follows the bidirectional inference
SetVAE is based on the bidirectional inference~\cite{sonderby2016ladder}, which is composed of the bottom-up encoder and top-down generator sharing the same dependency structure.
In this framework, the inference network forms the approximate posterior by merging bottom-up information from data with the top-down information from the generative prior.
We construct the encoder using a stack of ISABs in Section~\ref{sec:settransformer}, and treat each of the projected set $\mathbf{h}$ as a deterministic encoding of data.
% Following \cite{sonderby2016ladder}, we share the parameters between the generative and inference networks.
%{\color{blue}discuss the general characteristics of bidirectional inference to be self-contained: bottom-up encoding with ISAB, top-down inference with ABL.}

\iffalse
{\color{OliveGreen}
Here, the inference model uses the same dependency structure to the top-down generator.
During bidirectional inference, the inference network forms the approximate posterior by merging a bottom-up information from data with top-down information from the generative prior.
This requires a bottom-up encoder that extracts information from data.
For the purpose, we employ a stack of ISAB in Section~\ref{sec:settransformer} and treat each projected set $\mathbf{h}$ as deterministic encoding of data.}
\fi

Our generator is composed of a stack of special layers called Attentive Bottleneck Layer (ABL), which extends the ISAB in Section~\ref{sec:settransformer} with the stochastic interaction with the latent variable.
Specifically, ABL processes a set at each layer of the generator as follows:
\begin{align}
    \text{ABL}_m(\mathbf{x}) &= \text{MAB}(\mathbf{x}, \text{FF}(\mathbf{z}))\in \mathbb{R}^{n\times d}\label{eqn:abp}\\
    \text{with}~~\mathbf{h} &= \text{MAB}(I, \mathbf{x})\in \mathbb{R}^{m\times d}\label{eqn:abl_bottleneck},
\end{align}
where $\text{FF}$ denotes a feed-forward layer and the latent variable $\mathbf{z}$ is derived from the projection $\mathbf{h}$.
% {\color{red}We provide an illustration in Section~\ref{appendix:abl} of appendix.}
For generation (Figure~\ref{fig:setvae_generation}), we sample $\mathbf{z}$ from the prior in Eq.~\eqref{eqn:normal_prior} by,
\begin{align}
    % \mathbf{z} &\sim \mathcal{N}(\mu, \sigma),~\text{where}\nonumber\\
    % &\mu, \sigma = \text{FF}(\mathbf{h})
    \mathbf{z} &\sim \mathcal{N}(\mu, \sigma)~\text{where}~\mu, \sigma = \text{FF}(\mathbf{h}).
    \label{eqn:abp_z_prior}
\end{align}
For inference (Figure~\ref{fig:setvae_inference}), we sample $\mathbf{z}$ from the posterior in Eq.~\eqref{eqn:normal_posterior} by,
\begin{align}
    % &\mathbf{z} \sim \mathcal{N}(\mu+\Delta\mu, \sigma\cdot\Delta\sigma),~\text{where}\nonumber\\
    % &\Delta\mu, \Delta\sigma = \text{FF}(\mathbf{h}+\mathbf{h}'),
&\mathbf{z} \sim \mathcal{N}(\mu+\Delta\mu, \sigma\cdot\Delta\sigma) \nonumber\\
&\text{where}~\Delta\mu, \Delta\sigma = \text{FF}(\mathbf{h}+\mathbf{h}_{\text{enc}}),
    \label{eqn:abp_z_posterior}
\end{align}
where $\mathbf{h}_{\text{enc}}$ is obtained from the corresponding ISAB layer of the bottom-up encoder.
Following \cite{sonderby2016ladder}, we share the parameters between the generative and inference networks.
% Section~\ref{appendix:abl} of the supplementary file describes in-depth analysis of ABL.
% The supplementary file illustrates ABL in detail.
A detailed illustration of ABL is in the supplementary file.

%{\color{blue} discuss that the deterministic and stochastic processes in ABL, and it is indeed similar to Ladder VAE and its variants.}
To generate a set, we first sample the initial elements $\mathbf{z}^{(0)}$ and the latent variable $\mathbf{z}^{(1)}$ from the prior $p(\mathbf{z}^{(0)})$ and $p(\mathbf{z}^{(1)})$, respectively. 
Given these inputs, the generator iteratively samples the subsequent latent variables $\mathbf{z}^{(l)}$ from the prior $p(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)})$ one by one at each layer of ABL, while processing the set conditioned on the sampled latent variable via Eq.~\eqref{eqn:abp}. 
The data $\mathbf{x}$ is then decoded elementwise from the final output.
\iffalse
{\color{OliveGreen}
During generation, the latent variables are sampled in top-down order. At level $l$, an $\textnormal{ABL}$ predicts the parameters of prior conditional $p(\mathbf{z}^{(l)}|\mathbf{z}^{(<l)})$. After sampling, the latent variable is treated as a conditioning input, supporting the top-down dependency to the next level.
This is analogous to combination of deterministic and stochastic features during top-down pass in \cite{kingma2017improving}.
After all latent variables are sampled, a data sample can be decoded elementwise from the final output.
}
\fi
% For inferring the latent variables from a data, the generative network is reused, preserving the top-down sampling order.
% In this case, the parameters of approximate posterior $q(\mathbf{z}_l|\mathbf{z}_{<l}, \mathbf{x})$ are produced by correcting the prior with bottom-up information from data.
% In \cite{sonderby2016ladder}, this information is Gaussian parameters to be directly mixed with the prior.
% We instead follow the approach of \cite{kingma2017improving}, where the bottom-up information is combined with top-down feature once more to produce the prior correction term.
% In SetVAE, the bottom-up information is a projected set from an ISAB in encoder stack.


\subsection{Analysis}
% \paragraph{Permutation Invariance and Equivariance}
\paragraph{Modeling Exchangeable Likelihood}
%{\color{blue}Discuss that our generator and inference networks are permutation invariant/equivariant. Related this to the last paragraph of Section 3.}
The architecture of SetVAE satisfies the invariance and equivariance criteria in Section~\ref{sec:method}.
% This is in part ...
This is, in part, achieved by producing latent variables from the projected sets of bottom-up ISAB and top-down ABL.
As the projected sets are permutation invariant to input (Section~\ref{sec:preliminary}), the latent variables $\mathbf{z}^{(1:L)}$ provide an invariant representation of the data.
Furthermore, due to permutation equivariance of ISAB, the top-down stack of ABLs produce an output equivariant to the initial set $\mathbf{z}^{(0)}$. This renders the decoding distribution $p(\mathbf{x}|\mathbf{z}^{(0)}, \mathbf{z}^{(1:L)})$ permutation equivariant to $\mathbf{z}^{(0)}$.
Consequently, the decoder of SetVAE induces an exchangeable model.


% \paragraph{Hierarchical Subset Encoding}
\cutparagraphup
\paragraph{Learning Coarse-to-Fine Dependency}
%{\color{blue}Discuss that how ABL poses a bottleneck and learns coarse-to-fine subset interaction.}
In SetVAE, both the ISAB and ABL project the input set $\mathbf{x}$ of cardinality $n$ to the projected set $\mathbf{h}$ of cardinality $m$ via multi-head attention (Eq.~\eqref{eqn:isab_bottleneck} and \eqref{eqn:abl_bottleneck}).
% In case of $m<n$, this projection functions as a bottleneck to the cardinality, and allows the model to discover interesting \emph{subset} dependencies across the set elements.
In the case of $m<n$, this projection functions as a bottleneck to the cardinality.
This allows the model to encode some features of $\mathbf{x}$ into the $\mathbf{h}$ and discover interesting \emph{subset} dependencies across the set elements.
Denoting $m_l$ as the bottleneck cardinality at layer $l$ (Figure~\ref{fig:overview}), we set $m_{l}<m_{l+1}$ to induce the model to discover coarse-to-fine dependency of the set, such as object parts.
% ... the size of network ...
Such bottleneck also effectively reduces network size, allowing our model to perform competitive or better than the prior arts with less than 30\% of their parameters.
% We will show that our model performs competitive or better than the prior arts with less than 30\% of parameters.
%Denoting $m_l$ as the bottleneck cardinality at layer $l$ (Figure~\ref{fig:overview}), we show that setting the $m_{l}<m_{l+1}$ for some layers makes our model discover coarse-to-fine dependency of the set, such as object parts.
%It also encourages the corresponding latent variable $\mathbf{z}^{(l)}$ to capture the factors of variations in subsets, and allows part-based manipulations in generation. 
% This coarse-to-fine dependency structure is a unique feature of SetVAE.
This coarse-to-fine structure is a unique feature of SetVAE.

% {\color{OliveGreen}
% By producing latent variables from projected sets in ISAB, an ABL views latent variables as a \textit{latent set} of fixed cardinality.
% If the input sets have larger cardinality, the latent set can serve as an bottleneck.
% In this case, it would be beneficial for the model to encode some amortized features into the latent set, such that each latent element governs multiple elements in a data instance that forms a subset relation.
% Such relations could include semantically meaningful object parts, a template of objects co-occurring frequently in a scene, cluster centers that define a dataset, \etc.

% Moreover, as ABLs in different hierarchy could have different latent set cardinality, SetVAE admits a multi-scale architecture such that latent sets at different levels represent a different \textit{resolution} of the input or output set.
% Combined with top-down dependency introduced by hierarchical modeling, more flexible subset representations could be learned.
% In SetVAE, we choose to impose a top-down increase in the latent cardinality.
% This could allow the model to learn coarse-to-fine subset representation that compose set data, in analogy to the multi-scale image generators \cite{sonderby2016ladder, vahdat2020nvae}.
% }

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[b]{0.17\textwidth}
%         \centering
%         \includegraphics[height=5.5cm]{figures/fig_hgen.pdf}
%         \caption{Generation}
%         \label{fig:setvae_generation}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[height=5.5cm]{figures/fig_hinference.pdf}
%         \caption{Inference}
%         \label{fig:setvae_inference}
%     \end{subfigure}
%     \caption{The hierarchical SetVAE. {\color{red} $\sim$ denotes sampling, and + denotes feature combining via addition.}
%     \shcmt{This figure needs to be polished.}
%     {\color{magenta} JH: I will draw this if you are busy.}
%     }
%     \vspace{-0.5cm}
% \label{fig:overview}
% \end{figure}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.17\textwidth}
        \centering
        %\includegraphics[height=5.5cm]{figures/fig-3-prior.pdf}
        \includegraphics[height=5.5cm]{figures/SetVAE_generation.pdf}
        \caption{Generation}
        \label{fig:setvae_generation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        %\includegraphics[height=5.5cm]{figures/fig-3-posterior.pdf}
        \includegraphics[height=5.5cm]{figures/SetVAE_inference.pdf}
        \caption{Inference}
        \label{fig:setvae_inference}
    \end{subfigure}
    \caption{The hierarchical SetVAE. %$\sim$ denotes sampling.
    $\mathcal{N}_{prior}$ denotes the prior (Eq.~\eqref{eqn:abp_z_prior}) and $\mathcal{N}_{post}$ denotes the posterior (Eq.~\eqref{eqn:abp_z_posterior}).
    }
    \vspace{-0.3cm}
\label{fig:overview}
\end{figure}

\subsection{Implementation Details}
\label{sec:implementation}
\cutsubsectiondown
This section discusses the implementation of SetVAE.
We leave comprehensive details on the supplementary file.

\cutparagraphup
\iffalse
\paragraph{PreLN.} 
We observe that the Layer Normalization (LN) in ISAB and ABL makes the training unstable and hurts the performance.
We find that moving LN before the multi-head attention and feedforward layer as suggested by \cite{xiong2020layer} greatly improves the stability and performance.
\fi

\cutparagraphup
\paragraph{Multi-Modal Prior.} 
Although a unimodal Gaussian is a typical choice for the initial element distribution $p(\mathbf{z}^{(0)}_i)$ \cite{kosiorek2020conditional, yang2019pointflow}, we find that the model converges significantly faster when we employ the multi-modal prior.
We use a mixture of Gaussians (MoG) with $K$ components:
\begin{equation}
    p(\mathbf{z}^{(0)}_i) = \sum_{k=1}^K{\pi_k\mathcal{N}(\mathbf{z}^{(0)}_i|\mu^{(0)}_k, \sigma^{(0)}_k)}.
    \label{eqn:prior_mog}
\end{equation}
% which (i) can approximate any distribution in theory if $N$ is sufficiently large, and (ii) parameters can be trained by reparameterization trick.
% We downscale all covariance by multiplying $\frac{1}{K}$ after random initialization.
% To guarantee that the top-down ABLs sees multiple modes at the beginning of training, we downscale all covariance by multiplying $\frac{1}{K}$ after random initialization.

\cutparagraphup
\paragraph{Normalizing Flows.} A simple extension for more expressive $p(\mathbf{z}^{(0)})$ is passing the sampled initial set through a number of normalizing flows \cite{rezende2016variational}.
We demonstrate that applying a number of planar flows $f(\mathbf{z}^{(0)}_i) = \mathbf{z}^{(0)}_i + \mathbf{u}h(\mathbf{w}^\mathrm{T}\mathbf{z}^{(0)}_i+b)$ on top of MoG enhances model performance.
Although the normalizing flow itself can model the multi-modal prior distribution without MoG in principle, we found that the model converges much faster with the multi-modal prior.

% In theory, using a sufficient number of flows should be enough to anneal a Gaussian into multiple modes.
% However, we empirically observed that with a unimodal Gaussian as $p(\mathbf{x}_0^i)$, the top-down ResABLs converges much faster, falling into a local optima that does not leverage the flexibility of normalizing flows.

\cutparagraphup
\paragraph{Likelihood.}
For the likelihood $p_\theta(\mathbf{x}|\mathbf{z})$, we may consider a Gaussian distribution centered at the reconstruction.
In case of point sets, we design the likelihood by
\begin{align}
    \mathcal{L}_\text{recon}(\mathbf{x}) &= -\log p_\theta(\mathbf{x}|\mathbf{z})  
    \nonumber\\
    &= -\frac{1}{2}  \textnormal{EMD}(\mathbf{x}, \hat{\mathbf{x}}) + \mathrm{const},
\end{align}
where $\textnormal{EMD}(\mathbf{x}, \hat{\mathbf{x}})$ is the Earth Mover's Distance (EMD) defined as
\[
\textnormal{EMD}(\mathbf{x}, \hat{\mathbf{x}}) = \min_{\pi} \| \mathbf{x}_i - \hat{\mathbf{x}}_{\pi(i)}\|_2^2.
\]
In other words, we measure the likelihood with the Gaussian at optimally permuted $\mathbf{x}$, and thus maximizing this likelihood is equivalent to minimizing the EMD between the data and the reconstruction. Unfortunately, directly maximizing this likelihood requires $O(n^3)$ computation due to the optimal matching. Instead, we choose the Chamfer Distance (CD) as a proxy reconstruction loss,
\begin{align}
    \lefteqn{\mathcal{L}_\text{recon}(\mathbf{x}) = \textnormal{CD}(\mathbf{x}, \hat{\mathbf{x}})} \nonumber\\
    &= \sum_{i} \min_j \| \mathbf{x}_i - \hat{\mathbf{x}}_j\|_2^2 + \sum_j \min_i \|\mathbf{x}_i - \hat{\mathbf{x}}_j\|_2^2.
    \label{eqn:reconstruction_cd}
\end{align}

The CD may not admit a direct interpretation as a negative log-likelihood of $p_\theta(\mathbf{x}|\mathbf{z})$, but shares the optimum with the EMD having a proper interpretation. 
By employing the CD for the reconstruction loss, we learn the VAE with a surrogate for the likelihood $p_\theta(\mathbf{x}|\mathbf{z})$.
CD requires $O(n^2)$ computation time, so is scalable to the moderately large sets.
% Note also that the CD should be scaled appropriately to match the likelihood induced by EMD, but here we are not particularly doing that because we are balancing the reconstruction loss and the KL loss with $\beta$ anyway.
% ... properly scaled ...
Note also that the CD should be scaled appropriately to match the likelihood induced by EMD.
We implicitly account for this by applying weights to KL divergence in our final objective function:
\begin{equation}
    \mathcal{L}_{\textnormal{HSVAE}}(\mathbf{x}) = \mathcal{L}_{\textnormal{recon}}(\mathbf{x}) + \beta\mathcal{L}_{\textnormal{KL}}(\mathbf{x}),
    \label{eqn:beta_vae_loss}
\end{equation}
where $\mathcal{L}_{\textnormal{KL}}(\mathbf{x})$ is the KL divergence in Eq.~\eqref{eqn:elbo_hierarchicalSetVAE}.
% {\color{blue} where is the part defining overall loss function? ($\mathcal{L}_\text{recon}(\mathbf{x}) + \beta \mathrm{KL}$})

% The resulting final objective is:
% \begin{equation}
%     \mathcal{L}_{\textnormal{SVAE}}'(\mathbf{x}) = \mathcal{L}_{\textnormal{recon}}(\mathbf{x}) + \beta\mathcal{L}_{\textnormal{KL}}(\mathbf{x})
% \end{equation}
% To stabilize the training and avoid posterior collapse, we simply add a discounting factor $\beta$ to the KL \cite{Higgins2017betaVAELB}.


% !TEX root = cvpr.tex


==> cvpr_draft/preliminaries.tex <==
% !TEX root = cvpr.tex
\section{Preliminaries}
\label{sec:preliminary}

\subsection{Permutation-Equivariant Set Generation}
\label{sec:equivariant}
% {\color{magenta} why superscript for the data index $i$? its quite confusing with exponents. I recommend write element indices as subscripts, and write the latent level as parenthesized superscript. e.g., $\mathbf{z}_i^{(\ell)}$}
% Denote a set as ...
Denote a set as $\mathbf{x} = \{\mathbf{x}_i\}_{i=1}^n \in \mathcal{X}^n$, where $n$ is the cardinality of the set and $\mathcal{X}$ represents the domain of each element $\mathbf{x}_i \in\mathbb{R}^d$.
In this paper, we represent $\mathbf{x}$ as a matrix $\mathbf{x} = [\mathbf{x}_1, ..., \mathbf{x}_n]^\mathrm{T} \in\mathbb{R}^{n\times d}$.
Note that any operation on a set should be invariant to the elementwise permutation and satisfy the two constraints of \textit{permutation invariance} and \textit{permutation equivariance}.
% Note that any operations in set should satisfy the two conditions: \textit{permutation invariance} or \textit{permutation equivariance}
% Note that the set is 
% As any operation on a set should not depend on the ordering, a constraint is given to available operations \cite{zaheer2017deep}: they should be \textit{permutation invariant} or \textit{permutation equivariant}.
\begin{defn}
A function $f:\mathcal{X}^n \rightarrow \mathcal{Y}$ is permutation invariant iff for any permutation $\pi(\cdot)$, $f(\pi(\mathbf{x}))= f(\mathbf{x})$.
\end{defn}
% \noindent\textbf{Definition 1.} \textit{A function $f:\mathcal{X}^n \rightarrow \mathcal{Y}$ is permutation invariant iff for any permutation $\pi(\cdot)$, $f(\pi(\mathbf{x}))= f(\mathbf{x})$.}
\begin{defn}
A function $f:\mathcal{X}^n \rightarrow \mathcal{Y}^n$ is permutation equivariant iff for any permutation $\pi(\cdot)$, $f(\pi(\mathbf{x}))=\pi( f(\mathbf{x}))$.
\end{defn}
%
In the context of generative modeling, the notion of permutation invariance translates into the exchangeability, requiring a joint distribution of the elements invariant with respect to the permutation.
%
\begin{defn}
A distribution for a set of random variables $\mathbf{x} = \{\mathbf{x}_i\}_{i=1}^n$ is exchangeable if for any permutation $\pi$,
$p(\mathbf{x}) = p(\pi(\mathbf{x}))$.
\end{defn}

An easy way to achieve exchangeability is to assume each element to be \emph{i.i.d.} and process a set of initial elements $\mathbf{z}^{(0)} = \{\mathbf{z}_i^{(0)}\}_{i=1}^n$ independently sampled from $p(\mathbf{z}_i^{(0)})$ with an elementwise function $f_{\textnormal{elem}}$ to get the $\mathbf{x}$:
\begin{equation}
    \mathbf{x} = \{\mathbf{x}_i\}_{i=1}^n \textnormal{ where } \mathbf{x}_i = f_{\textnormal{elem}} (\mathbf{z}_i^{(0)})
\end{equation}

However, assuming elementwise independence poses a limit in modeling interactions between set elements.
An alternative direction is to process $\mathbf{z}^{(0)}$ with a permutation-equivariant function $f_{\textnormal{equiv}}$ to get the $\mathbf{x}$:
\begin{equation}
    \mathbf{x} = \{\mathbf{x}_i\}_{i=1}^n = f_{\textnormal{equiv}}(\{\mathbf{z}_i^{(0)}\}_{i=1}^n).
\end{equation}

We refer to this approach as the \textit{permutation-equivariant generative framework}.
As the likelihood of $\mathbf{x}$ does not depend on the order of its elements (because elements of $\mathbf{z}^{(0)}$ are i.i.d.), this approach achieves exchangeability.

% Permutation-equivariant generative framework can account for the intermediate element interactions, and has been adopted in recent works for set autoencoding \cite{zhang2020deep, kosiorek2020conditional}, often with equivariant neural networks \cite{zaheer2017deep, lee2019set} as $f_{\textnormal{equiv}}$.

% \subsection{Set Transformer}
\subsection{Permutation-Equivariant Set Encoding}
\label{sec:settransformer}
% Encoder-decoder architectures for image or sequence cannot be directly applied to sets due to the requirement for a permutation \textit{invariant} encoder and a permutation \textit{equivariant} decoder \cite{zaheer2017deep}.
% As a solution, Set Transformer (ST) \cite{lee2019set} provides attentive modules that model pairwise interaction between set elements while preserving invariance or equivariance.
% To design a permutation-equivariant operations over set
To design permutation-equivariant operations over a set, Set Transformer~\cite{lee2019set} provides attentive modules that model pairwise interaction between set elements while preserving invariance or equivariance.
This section introduces two essential modules in the Set Transformer. 
\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=0.6\textwidth]{figures/fig_mab.pdf}
        % \caption{Multihead Attention Block (MAB) with two sets $Q$ and $V$ as input. Cardinality of $Q$ and $V$ are arbitrary.}
        \caption{MAB}
        \label{fig:mab}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=0.6\textwidth]{figures/fig_isab2.pdf}
        \caption{ISAB}
        % \caption{Induced Set Attention Block (ISAB). Fixed cardinality $m$ is marked red. Cardinality of input $\mathbf{x}$ is arbitrary.}
        \label{fig:isab}
    \end{subfigure}
    \caption{Illustration of Multihead Attention Block (MAB) and Induced Set Attention Block (ISAB).}
\label{fig:st}
\vspace{-0.5cm}
\end{figure}

% As a building block, Set Transformer defines Multihead Attention Block (MAB) which accepts a query set $Q=\{q_i\}_{i=1}^{n_q} \in \mathbb{R}^{n_q\times d}$ and a value set $V=\{v_j\}_{j=1}^{n_v} \in \mathbb{R}^{n_v\times d}$ of any cardinality and performs the following (Figure \ref{fig:mab}):
First, Multihead Attention Block (MAB) takes the query and value sets, $Q\in \mathbb{R}^{n_q\times d}$ and  $V\in \mathbb{R}^{n_v\times d}$, respectively, and performs the following transformation (Figure \ref{fig:mab}):
\begin{align}
    \textnormal{MAB}(Q, V) = \textnormal{LN}(\mathbf{a} + \textnormal{FF}(\mathbf{a})) \in \mathbb{R}^{n_q\times d},~~~~ \label{eqn:MAB}\\
    \textnormal{where }
    \mathbf{a} = \textnormal{LN}(Q + \textnormal{Multihead}(Q, V, V)) \in \mathbb{R}^{n_q\times d},\label{eqn:MAB_att}
\end{align}
where FF denotes elementwise feedforward layer, Multihead denotes multi-head attention~\cite{vaswani2017attention}, and LN denotes layer normalization \cite{lee2019set}.
Note that the output of Eq.~\eqref{eqn:MAB} is permutation equivariant to $Q$ and permutation invariant to $V$.

% Now, we define the Induced Set Attention Block (ISAB) with two MABs.
Based on MAB, Induced Set Attention Block (ISAB) processes the input set $\mathbf{x}\in\mathbb{R}^{n\times d}$ using a 
smaller set of inducing points $I\in \mathbb{R}^{m\times d}~(m<n)$ by (Figure \ref{fig:isab}):
\begin{align}
    \textnormal{ISAB}_m(\mathbf{x}) &= \textnormal{MAB}(\mathbf{x}, \mathbf{h}) \in \mathbb{R}^{n\times d}, \\
    \textnormal{where }\mathbf{h} &= \textnormal{MAB}(I, \mathbf{x}) \in \mathbb{R}^{m\times d}\label{eqn:isab_bottleneck}.
\end{align}
%
% The ISAB first transforms the input set $\mathbf{x}$ into $\mathbf{h}$ by attending from $I$ with a lower cardinality $m$, then projects it back to the original cardinality $n$ by attending it to $\mathbf{x}$.
% Then, $\mathbf{h}$ is again attended to $\mathbf{x}$ to produce the output of $n$ elements (we call this the \textit{backprojecting attention}).
% The ISAB first transforms the input set $\mathbf{x}$ into $\mathbf{h}$ by attending from $I$ (we call this the \textit{projecting attention}).
% The resulting $\mathbf{h}$ is a permutation invariant projection of $\mathbf{x}$ to a lower cardinality $m$.
% Then, $\mathbf{h}$ is again attended to $\mathbf{x}$ to produce the output of $n$ elements (we call this the \textit{backprojecting attention}).
The ISAB first transforms the input set $\mathbf{x}$ into $\mathbf{h}$ by attending from $I$.
The resulting $\mathbf{h}$ is a permutation invariant projection of $\mathbf{x}$ to a lower cardinality $m$.
Then, $\mathbf{x}$ again attends to $\mathbf{h}$ to produce the output of $n$ elements.
As a result, ISAB is permutation equivariant to $\mathbf{x}$.

% \noindent\textbf{Property 1.} \textit{In $\textnormal{ISAB}_m(\mathbf{x})$, $\mathbf{h}$ is permutation invariant to $\mathbf{x}$.}
% \noindent\textbf{Property 2.} \textit{$\textnormal{ISAB}_m(\mathbf{x})$ is permutation equivariant to $\mathbf{x}$.}
\begin{property}
In $\textnormal{ISAB}_m(\mathbf{x})$, $\mathbf{h}$ is permutation invariant to $\mathbf{x}$.
\end{property}
\begin{property}
\vspace{-0.2cm}
$\textnormal{ISAB}_m(\mathbf{x})$ is permutation equivariant to $\mathbf{x}$.
\end{property}


==> cvpr_draft/related_work.tex <==
% !TEX root = cvpr.tex
\section{Related Work}
\label{sec:related}
\input{table} % belongs to experiments, here for formatting
%\cutparagraphup
\paragraph{Set generative modeling.} SetVAE is closely related to recent works on permutation-equivariant set prediction \cite{zhang2020deep, kosiorek2020conditional, carion2020endtoend, locatello2020objectcentric, li2020exchangeable}.
Closest to our approach is the autoencoding TSPN \cite{kosiorek2020conditional} that uses a stack of ISABs \cite{lee2019set} to predict a set from randomly initialized elements.
However, TSPN does not allow sampling, as it uses a pooling-based deterministic set encoding (FSPool) \cite{zhang2020fspool} for reconstruction.
SetVAE instead discards FSPool and access projected sets in ISAB directly, which allows an efficient variational inference and a direct extension to hierarchical multi-scale latent.

Our approach differs from previous generative models treating each element \emph{i.i.d.} and processing a random initial set with an elementwise function \cite{edwards2017neural, yang2019pointflow, kim2020softflow}.
Notably, PointFlow \cite{yang2019pointflow} uses a continuous normalizing flow (CNF) to process a 3D Gaussian point cloud into an object.
% ... with attention ...
However, assuming elementwise independence could pose a limit in modeling complex element interactions.
Also, CNF requires the invertibility of the generative model, which could further limit its expressiveness.
SetVAE resolves this problem by adopting permutation equivariant ISAB that models inter-element interactions via attention, and a hierarchical VAE framework with flexible latent dependency.

We emphasize that SetVAE could also be extended to generative modeling of sparse object bounding boxes \cite{hong2018inferring, li2019grains, purkait2020sgvae} that often relies on specific ordering or alignment heuristics, which we leave for future work.

\cutparagraphup
\paragraph{Hierarchical VAE.}
% We borrow the statistical models (hierarchical prior and approximate posterior, ELBO, \etc.) from prior works on hierarchical extension of image VAE, namely Ladder-VAE \cite{sonderby2016ladder}, IAF-VAE \cite{kingma2017improving}, and NVAE \cite{vahdat2020nvae}.
% Our model is built upon the statistical models from prior works on hierarchical extension of image VAE, namely Ladder-VAE \cite{sonderby2016ladder}, IAF-VAE \cite{kingma2017improving}, and NVAE \cite{vahdat2020nvae}.
Our model is built upon the prior works on hierarchical VAEs for images, such as Ladder-VAE \cite{sonderby2016ladder}, IAF-VAE \cite{kingma2017improving}, and NVAE \cite{vahdat2020nvae}.
% Our model is built upon the statistical models from prior works on hierarchical extension of image VAE, namely Ladder-VAE \cite{sonderby2016ladder}, IAF-VAE \cite{kingma2017improving}, and NVAE \cite{vahdat2020nvae}.
To model long-range pixel correlations in images, these models organize latent variables at each hierarchy as images while gradually increasing their resolution via upsampling.
%StyleGAN \cite{karras2019stylebased} adopts a similar approach as well.
However, the requirement for permutation equivariance has prevented applying multi-scale approaches to sets.
ABLs in SetVAE solve this problem by defining latent variables in the projected scales of each hierarchy.


==> cvpr_draft/table.tex <==
% !TEX root = cvpr.tex

% without JSD
\begin{table*}[htbp!]
\caption{Comparison against the state-of-the-art generative models. $\uparrow$: the higher the better.
$\downarrow$: the lower the better. The best scores are highlighted in bold. MMD-CD is scaled by $10^3$, and MMD-EMD by $10^2$.}
\footnotesize
\begin{adjustbox}{width=1\textwidth}
\label{table:pointeval}
\centering
\begin{tabular}{clccccccccc}
\Xhline{2\arrayrulewidth}
\\[-1em]& & \multicolumn{2}{c}{\# Parameters (M)} & \multicolumn{2}{c}{MMD($\downarrow$)} & \multicolumn{2}{c}{COV($\%$,$\uparrow$)} &  \multicolumn{2}{c}{1-NNA($\%$,$\downarrow$)} \\
\\[-1em]\cline{3-4} \cline{5-6} \cline{7-8} \cline{9-10}
\\[-1em]Category & Model & Full & Gen & CD & EMD & CD & EMD & CD & EMD \\
\\[-1em]\Xhline{2\arrayrulewidth}
\\[-1em]\multirow{7}{*}{\shortstack{Airplane}}
    & l-GAN (CD)\cite{yang2019pointflow}    & 1.97 & 1.71 & 0.239 & 4.27 & 43.21 & 21.23 & 86.30 & 97.28\\
    & l-GAN (EMD)\cite{yang2019pointflow}   & 1.97 & 1.71 & 0.269 & 3.29 & 47.90 & \textbf{50.62} & 87.65 & 85.68\\
    & PC-GAN\cite{yang2019pointflow}        & 9.14 & 1.52 & 0.287 & 3.57 & 36.46 & 40.94 & 94.35 & 92.32\\
    & PointFlow\cite{yang2019pointflow}     & 1.61 & 1.06 & 0.217 & \textbf{3.24} & 46.91 & 48.40 & \textbf{75.68} & \textbf{75.06}\\
% Temperature 1.0
    & SetVAE (Ours) & \textbf{0.53} & \textbf{0.28} & \textbf{0.216} & 3.26 & \textbf{50.12} & 46.67 & 78.40 & 84.07 \\
    \\[-1em]\cline{2-10}
    \\[-1em]& Training set & - & - & 0.226 & 3.08 & 42.72 & 49.14 & 70.62 & 67.53 \\
\\[-1em]\Xhline{2\arrayrulewidth}
\\[-1em]\multirow{7}{*}{\shortstack{Chair}}
    & l-GAN (CD)\cite{yang2019pointflow} & 1.97 & 1.71 & 2.46 & 8.91 & 41.39 & 25.68 & 64.43 & 85.27\\
    & l-GAN (EMD)\cite{yang2019pointflow} & 1.97 & 1.71 & 2.61 & \textbf{7.85} & 40.79 & 41.69 & 64.73 & 65.56\\
    & PC-GAN\cite{yang2019pointflow} & 9.14 & 1.52 & 2.75 & 8.20 & 36.50 & 38.98 & 76.03 & 78.37\\
    & PointFlow\cite{yang2019pointflow} & 1.61 & 1.06 & \textbf{2.42} & 7.87 & 46.83 & 46.98 & 60.88 & \textbf{59.89}\\
% Temp 1.3
    & SetVAE (Ours) & \textbf{0.53} & \textbf{0.28} & 2.61 & 8.18 & \textbf{50.91} & \textbf{50.76} & \textbf{56.65} & 62.16\\
    \\[-1em]\cline{2-10}
    \\[-1em]& Training set & - & - & 1.92 & 7.38 & 57.25 & 55.44 & 59.67 & 58.46 \\
\\[-1em]\Xhline{2\arrayrulewidth}
\\[-1em]\multirow{7}{*}{\shortstack{Car}}
    & l-GAN (CD)\cite{yang2019pointflow} & 1.97 & 1.71 & 1.55 & 6.25 & 38.64 & 18.47 & 63.07 & 88.07\\
    & l-GAN (EMD)\cite{yang2019pointflow} & 1.97 & 1.71 & 1.48 & 5.43 & 39.20 & 39.77 & 69.74 & 68.32\\
    & PC-GAN\cite{yang2019pointflow} & 9.14 & 1.52 & 1.12 & 5.83 & 23.56 & 30.29 & 92.19 & 90.87\\
    & PointFlow\cite{yang2019pointflow} & 1.61 & 1.06 & 0.91 & 5.22 & 44.03 & 46.59 & 60.65 & \textbf{62.36} \\
% Using Temp 1.3
    & SetVAE (Ours) & \textbf{0.53} & \textbf{0.28} & \textbf{0.89} & \textbf{5.09} & \textbf{47.44} & \textbf{50.57} & \textbf{59.09} & 63.92 \\
    \\[-1em]\cline{2-10}
    \\[-1em]& Training set & - & - & 1.03 & 5.33 & 48.30 & 51.42 & 57.39 & 53.27 \\
\\[-1em]\Xhline{2\arrayrulewidth}
\end{tabular}
\end{adjustbox}
\end{table*}

% backup
\iffalse
\begin{table*}[htbp!]
\caption{Comparison against the state-of-the-art generative models. $\uparrow$: the higher the better.
$\downarrow$: the lower the better. The best scores are highlighted in bold. JSD is scaled by $10^2$, MMD-CD by $10^3$, and MMD-EMD by $10^2$.}
\begin{adjustbox}{width=1\textwidth}
\label{table:pointeval}
\centering
\begin{tabular}{clcccccccccc}
\Xhline{2\arrayrulewidth}
\\[-1em]& & \multicolumn{2}{c}{\# Parameters (M)} & \multirow{2}{*}{JSD($\downarrow$)} & \multicolumn{2}{c}{MMD($\downarrow$)} & \multicolumn{2}{c}{COV($\%$,$\uparrow$)} &  \multicolumn{2}{c}{1-NNA($\%$,$\downarrow$)} \\
\\[-1em]\cline{3-4} \cline{6-7} \cline{8-9} \cline{10-11}
\\[-1em]Category & Model & Full & Gen & & CD & EMD & CD & EMD & CD & EMD \\
\\[-1em]\Xhline{2\arrayrulewidth}
\\[-1em]\multirow{7}{*}{\shortstack{Airplane}}
    & l-GAN (CD)\cite{yang2019pointflow}    & 1.97 & 1.71 & 4.62 & 0.239 & 4.27 & 43.21 & 21.23 & 86.30 & 97.28\\
    & l-GAN (EMD)\cite{yang2019pointflow}   & 1.97 & 1.71 & 3.61 & 0.269 & 3.29 & 47.90 & \textbf{50.62} & 87.65 & 85.68\\
    & PC-GAN\cite{yang2019pointflow}        & 9.14 & 1.52 & 4.63 & 0.287 & 3.57 & 36.46 & 40.94 & 94.35 & 92.32\\
    & PointFlow\cite{yang2019pointflow}     & 1.61 & 1.06 & 4.92 & 0.217 & \textbf{3.24} & 46.91 & 48.40 & \textbf{75.68} & \textbf{75.06}\\
%    & EBP\cite{yang2020energybased}     & - & - & 3.92 & 0.240 & 3.22 & 49.38 & 51.60 & - & - \\
% Temperature 1.0
    & SetVAE (Ours) & \textbf{0.53} & \textbf{0.28} & {\textbf{3.32}} & \textbf{0.216} & 3.26 & \textbf{50.12} & 46.67 & 78.40 & 84.07 \\
    % & SetVAE (PostLN) & \textbf{0.53} & \textbf{0.28} & {\color{red}4.07} & 0.222 & 3.29 & \textbf{49.88} & 44.44 & 78.40 & 83.46 \\
    \\[-1em]\cline{2-11}
    \\[-1em]& Training set & - & - & 6.61 & 0.226 & 3.08 & 42.72 & 49.14 & 70.62 & 67.53 \\
\\[-1em]\Xhline{2\arrayrulewidth}
\\[-1em]\multirow{7}{*}{\shortstack{Chair}}
    & l-GAN (CD)\cite{yang2019pointflow} & 1.97 & 1.71 & 4.59 & 2.46 & 8.91 & 41.39 & 25.68 & 64.43 & 85.27\\
    & l-GAN (EMD)\cite{yang2019pointflow} & 1.97 & 1.71 & 2.27 & 2.61 & \textbf{7.85} & 40.79 & 41.69 & 64.73 & 65.56\\
    & PC-GAN\cite{yang2019pointflow} & 9.14 & 1.52 & 3.90 & 2.75 & 8.20 & 36.50 & 38.98 & 76.03 & 78.37\\
    & PointFlow\cite{yang2019pointflow} & 1.61 & 1.06 & \textbf{1.74} & \textbf{2.42} & 7.87 & 46.83 & 46.98 & 60.88 & \textbf{59.89}\\
%    & EBP\cite{yang2020energybased} & - & - & 1.53 & 2.59 & 7.92 & 47.73 & 49.84 & - & - \\
% Temp 1.3
    & SetVAE (Ours) & \textbf{0.53} & \textbf{0.28} & 1.92 & 2.60 & 8.17 & \textbf{49.70} & \textbf{47.13} & \textbf{58.16} & 62.61\\
    \\[-1em]\cline{2-11}
    \\[-1em]& Training set & - & - & 1.50 & 1.92 & 7.38 & 57.25 & 55.44 & 59.67 & 58.46 \\
\\[-1em]\Xhline{2\arrayrulewidth}
\\[-1em]\multirow{7}{*}{\shortstack{Car}}
    & l-GAN (CD)\cite{yang2019pointflow} & 1.97 & 1.71 & 4.43 & 1.55 & 6.25 & 38.64 & 18.47 & 63.07 & 88.07\\
    & l-GAN (EMD)\cite{yang2019pointflow} & 1.97 & 1.71 & 2.21 & 1.48 & 5.43 & 39.20 & 39.77 & 69.74 & 68.32\\
    & PC-GAN\cite{yang2019pointflow} & 9.14 & 1.52 & 5.85 & 1.12 & 5.83 & 23.56 & 30.29 & 92.19 & 90.87\\
    & PointFlow\cite{yang2019pointflow} & 1.61 & 1.06 & \textbf{0.87} & 0.91 & 5.22 & 44.03 & 46.59 & 60.65 & \textbf{62.36} \\
%    & EBP\cite{yang2020energybased} & - & - & \textbf{0.78} & 0.95 & 5.24 & \textbf{51.99} & 51.70 & - & - \\
% Using Temperature 1.2 for CD, 1.0 for EMD (Will be updated)
%    & SetVAE (ours) & \textbf{0.53} & \textbf{0.28} & 1.04 & \textbf{0.89} & {\color{red}\textbf{5.18}} & \textbf{51.42} & {\color{red}42.90} & \textbf{59.51} & {\color{red}65.48} \\
% Using Temp 1.3
    & SetVAE (Ours) & \textbf{0.53} & \textbf{0.28} & 0.98 & \textbf{0.89} & \textbf{5.09} & \textbf{47.44} & \textbf{50.57} & \textbf{59.09} & 63.92 \\
    \\[-1em]\cline{2-11}
    \\[-1em]& Training set & - & - & 0.86 & 1.03 & 5.33 & 48.30 & 51.42 & 57.39 & 53.27 \\
\\[-1em]\Xhline{2\arrayrulewidth}
\end{tabular}
\end{adjustbox}
\end{table*}
\fi
